Understanding Regularization to Visualize Convolutional Neural Networks

Variational methods for revealing visual concepts learned by convolutional neural networks have gained significant attention during the last years. Being based on noisy gradients obtained via back-propagation such methods require the application of regularization strategies. We present a mathematical framework unifying previously employed regularization methods. Within this framework, we propose a novel technique based on Sobolev gradients which can be implemented via convolutions and does not require specialized numerical treatment, such as total variation regularization. The experiments performed on feature inversion and activation maximization demonstrate the benefit of a unified approach to regularization, such as sharper reconstructions via the proposed Sobolev filters and a better control over reconstructed scales.

==> fig_activationmax.tex <==
\begin{figure}%
\centering
\subfloat[VGG19]{%
\label{fig:AMVGG19}%
\begin{minipage}{0.48\textwidth}
\begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.49\textwidth]{artwork/vgg19_fluid_None.png}
\put(5,5){\textcolor{black}{fluid}}
\end{overpic}
\hfill
\begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.49\textwidth]{artwork/vgg19_elastic_None.png}
\put(5,5){\textcolor{black}{elastic}}
\end{overpic}
\\[0.2em]
\begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.49\textwidth]{artwork/vgg19_ascend_TV.png}
\put(5,5){\textcolor{black}{TV}}
\end{overpic}
\hfill
\begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.49\textwidth]{artwork/vgg19_demons_None.png}
\put(5,5){\textcolor{black}{demons}}
\end{overpic}
\end{minipage}
}%
\hfill
\subfloat[ResNet-50]{%
\label{fig:AMResNet50}%
\begin{minipage}{0.48\textwidth}
\begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.49\textwidth]{artwork/resnet_fluid_None.png}
\put(5,5){\textcolor{black}{fluid}}
\end{overpic}
\hfill
\begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.49\textwidth]{artwork/resnet_elastic_None.png}
\put(5,5){\textcolor{black}{elastic}}
\end{overpic}
\\[0.2em]
\begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.49\textwidth]{artwork/resnet_ascend_TV.png}
\put(5,5){\textcolor{black}{TV}}
\end{overpic}
\hfill
\begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.49\textwidth]{artwork/resnet_demons_None.png}
\put(5,5){\textcolor{black}{demons}}
\end{overpic}
\end{minipage}
}%
\\
\subfloat[InceptionV3]{%
\label{fig:AMInceptionV3}%
\begin{minipage}{0.48\textwidth}
\begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.49\textwidth]{artwork/inception_fluid_None.png}
\put(5,5){\textcolor{black}{fluid}}
\end{overpic}
\hfill
\begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.49\textwidth]{artwork/inception_elastic_None.png}
\put(5,5){\textcolor{black}{elastic}}
\end{overpic}
\\[0.2em]
\begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.49\textwidth]{artwork/inception_ascend_TV.png}
\put(5,5){\textcolor{black}{TV}}
\end{overpic}
\hfill
\begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.49\textwidth]{artwork/inception_demons_None.png}
\put(5,5){\textcolor{black}{demons}}
\end{overpic}
\end{minipage}
}%
\hfill
\subfloat[InceptionResNetV2]{%
\label{fig:AMInceptionDenseNetV2}%
\begin{minipage}{0.48\textwidth}
\begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.49\textwidth]{artwork/inc_res_fluid_None.png}
\put(5,5){\textcolor{black}{fluid}}
\end{overpic}
\hfill
\begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.49\textwidth]{artwork/inc_res_elastic_None.png}
\put(5,5){\textcolor{black}{elastic}}
\end{overpic}
\\[0.2em]
\begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.49\textwidth]{artwork/inc_res_ascend_TV.png}
\put(5,5){\textcolor{black}{TV}}
\end{overpic}
\hfill
\begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.49\textwidth]{artwork/inc_res_demons_None.png}
\put(5,5){\textcolor{black}{demons}}
\end{overpic}
\end{minipage}
}%
\\
\subfloat[DenseNet]{%
\label{fig:AMDenseNet}%
\begin{minipage}{0.48\textwidth}
\begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.49\textwidth]{artwork/densenet121_fluid_None.png}
\put(5,5){\textcolor{black}{fluid}}
\end{overpic}
\hfill
\begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.49\textwidth]{artwork/densenet121_elastic_None.png}
\put(5,5){\textcolor{black}{elastic}}
\end{overpic}
\\[0.2em]
\begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.49\textwidth]{artwork/densenet121_ascend_TV.png}
\put(5,5){\textcolor{black}{TV}}
\end{overpic}
\hfill
\begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.49\textwidth]{artwork/densenet121_demons_None.png}
\put(5,5){\textcolor{black}{demons}}
\end{overpic}
\end{minipage}
}%
\hfill
\subfloat[NasNet]{%
\label{fig:AMNasNet}%
\begin{minipage}{0.48\textwidth}
\begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.49\textwidth]{artwork/NASNet_fluid_None.png}
\put(5,5){\textcolor{black}{fluid}}
\end{overpic}
\hfill
\begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.49\textwidth]{artwork/NASNet_elastic_None.png}
\put(5,5){\textcolor{black}{elastic}}
\end{overpic}
\\[0.2em]
\begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.49\textwidth]{artwork/NASNet_ascend_TV.png}
\put(5,5){\textcolor{black}{TV}}
\end{overpic}
\hfill
\begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.49\textwidth]{artwork/NASNet_demons_None.png}
\put(5,5){\textcolor{black}{demons}}
\end{overpic}
\end{minipage}
}%
\\
\caption{\textbf{Qualitative Comparison for Activation Maximization:} Comparison of the three derived optimization schemes to TV regularization for various images and network architectures pre-trained on ImageNet. VGG: Barnspider, ResNet: Candle, InceptionV3: Starfish, InceptionResNetV2: Fire-Salamander, DenseNet: Volleyball, NasNet: Hammerhead}
\end{figure}

==> fig_activationmax_new.tex <==
% !TEX root = ieee_tip.tex
\begin{figure*}[p]
\def\thisfigwidth{0.31\textwidth}
	\begin{minipage}[t]{1\textwidth}
            \begingroup
			%\parfillskip=0pt
			\hfill
			\begin{minipage}[c]{0.04\textwidth}
				\begin{turn}{90}\small{VGG19}\end{turn}\hfill
			\end{minipage}%
			\begin{minipage}[c]{0.96\textwidth}
				\begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.24\textwidth]{artwork/vgg19_ascend_TV.png}
                \put(5,5){\textcolor{white}{TV}}
                \end{overpic}
                \hfill
                \begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.24\textwidth]{artwork/vgg19_fluid_None.png}
                \put(5,5){\textcolor{white}{fluid}}
                \end{overpic}
                \begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.24\textwidth]{artwork/vgg19_elastic_None.png}
                \put(5,5){\textcolor{white}{elastic}}
                \end{overpic}
                \hfill
                \begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.24\textwidth]{artwork/vgg19_demons_None.png}
                \put(5,5){\textcolor{white}{demons}}
                \end{overpic}
                \\[0.2em]
                \begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.24\textwidth]{artwork/vgg19_ascend_TV_scale.png}
                \put(5,5){\textcolor{white}{TV + octave}}
                \end{overpic}
                \hfill
                \begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.24\textwidth]{artwork/vgg19_fluid_None_scale.png}
                \put(5,5){\textcolor{white}{fluid + octave}}
                \end{overpic}
                \begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.24\textwidth]{artwork/vgg19_elastic_None_scale.png}
                \put(5,5){\textcolor{white}{elastic + octave}}
                \end{overpic}
                \hfill
                \begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.24\textwidth]{artwork/vgg19_demons_None_scale.png}
                \put(5,5){\textcolor{white}{demons + octave}}
                \end{overpic}					
			\end{minipage}%			
			\par\endgroup
			\vspace{2ex}
			\begingroup
			%\parfillskip=0pt
			\hfill
			\begin{minipage}[c]{0.04\textwidth}
				\begin{turn}{90}\small{ResNet}\end{turn}
				%\hfill
			\end{minipage}%
				\begin{minipage}[c]{0.96\textwidth}
				\begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.24\textwidth]{artwork/resnet_ascend_TV.png}
                \put(5,5){\textcolor{white}{TV}}
                \end{overpic}
                \hfill
                \begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.24\textwidth]{artwork/resnet_fluid_None.png}
                \put(5,5){\textcolor{white}{fluid}}
                \end{overpic}
                \begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.24\textwidth]{artwork/resnet_elastic_None.png}
                \put(5,5){\textcolor{white}{elastic}}
                \end{overpic}
                \hfill
                \begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.24\textwidth]{artwork/resnet_demons_None.png}
                \put(5,5){\textcolor{white}{demons}}
                \end{overpic}
                \\[0.2em]
                \begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.24\textwidth]{artwork/resnet_ascend_TV_scale.png}
                \put(5,5){\textcolor{white}{TV + octave}}
                \end{overpic}
                \hfill
                \begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.24\textwidth]{artwork/resnet_fluid_None_scale.png}
                \put(5,5){\textcolor{white}{fluid + octave}}
                \end{overpic}
                \begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.24\textwidth]{artwork/resnet_elastic_None_scale.png}
                \put(5,5){\textcolor{white}{elastic + octave}}
                \end{overpic}
                \hfill
                \begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.24\textwidth]{artwork/resnet_demons_None_scale.png}
                \put(5,5){\textcolor{white}{demons + octave}}
                \end{overpic}					
			\end{minipage}%	
			\par\endgroup
						\vspace{2ex}
		    \begingroup
		    %\parfillskip=0pt
		    \hfill
		    \begin{minipage}[c]{0.04\textwidth}
		    	\begin{turn}{90}\small{DenseNet-121}\end{turn}
		    \end{minipage}%
				\begin{minipage}[c]{0.96\textwidth}
				\begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.24\textwidth]{artwork/dense_ascend_TV.png}
                \put(5,5){\textcolor{white}{TV}}
                \end{overpic}
                \hfill
                \begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.24\textwidth]{artwork/dense_fluid_None.png}
                \put(5,5){\textcolor{white}{fluid}}
                \end{overpic}
                \begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.24\textwidth]{artwork/dense_elastic_None.png}
                \put(5,5){\textcolor{white}{elastic}}
                \end{overpic}
                \hfill
                \begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.24\textwidth]{artwork/dense_demons_None.png}
                \put(5,5){\textcolor{white}{demons}}
                \end{overpic}
                \\[0.2em]
                \begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.24\textwidth]{artwork/dense_ascend_TV_scale.png}
                \put(5,5){\textcolor{white}{TV + octave}}
                \end{overpic}
                \hfill
                \begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.24\textwidth]{artwork/dense_fluid_None_scale.png}
                \put(5,5){\textcolor{white}{fluid + octave}}
                \end{overpic}
                \begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.24\textwidth]{artwork/dense_elastic_None_scale.png}
                \put(5,5){\textcolor{white}{elastic + octave}}
                \end{overpic}
                \hfill
                \begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.24\textwidth]{artwork/dense_demons_None_scale.png}
                \put(5,5){\textcolor{white}{demons + octave}}
                \end{overpic}					
			\end{minipage}%	
		    \par\endgroup
	\end{minipage}		
	\vspace{1.5ex}
	\caption{\textbf{Comparison} }
	\label{fig:comparison}
\end{figure*}

==> fig_comp_to_NN_reg.tex <==
\begin{figure}
%
\centering
%
\begin{minipage}{1.0\textwidth}
\begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.32\textwidth]{artwork/dummy.png}
\put(5,5){\textcolor{black}{Sobolev fluid}}
\end{overpic}
\hfill
\begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.32\textwidth]{artwork/dummy.png}
\put(5,5){\textcolor{black}{TV}}
\end{overpic}
\hfill
\begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.32\textwidth]{artwork/dummy.png}
\put(5,5){\textcolor{black}{Deep prior}}
\end{overpic}
\end{minipage}\\[0.5em]
%
\begin{minipage}{1.0\textwidth}
\begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.49\textwidth]{artwork/dummy.png}
\put(5,5){\textcolor{black}{Deep prior + Sobolev fluid}}
\end{overpic}
\hfill
\begin{overpic}[clip,trim=0cm 0cm 0cm 0cm,width=0.49\textwidth]{artwork/dummy.png}
\put(5,5){\textcolor{black}{Deep prior + TV}}
\end{overpic}
%
\end{minipage}
%
\label{fig:SobolevGaussian}
\caption{\textbf{Comparison to Deep Prior:} Reconstruction from Alex network pre-trained on ImageNet. \todo{interpretation}}
\end{figure}

==> stuff.tex <==
we start by considering the general form of such a problem:
\begin{equation}
    \min_{u\in\mathcal{F}}D(u,\theta) + \lambda R(u),
    \label{eqn:varProb}
\end{equation}
where $u$ is the pre-image to be computed, $\mathcal{F}$ denotes the function space in which $u$ is supposed to lie, $D$ is a data term that measures how well $u$ fulfills a certain task specified by set of parameters $\theta$, $R$ is a regularization term that only depends on $u$, and $\lambda>0$ is a parameter to control the trade-off between data fidelity and regularity.
If we consider the task of inversion, \ie reconstructing an image from a the features of a certain layer, $u$ would be the reconstructed image, $\theta$ would comprise the weights of the network and the features of the original image, $R$ could be the total variation and $\mathcal{F}$ could be the space of square integrable functions $L^2$.
Taking a closer look at \eqref{eqn:varProb}, one can identify two ways of regularizing such a variational problem:
\begin{enumerate}
    \item \textit{explicit regularization} via the regularizer $R$, \ie choosing an appropriate regularization term and adding it to the data term, and
    \item \textit{implicit regularization} via the function space $\mathcal{F}$, \ie choosing a sufficiently regular function space or changing the metric in this function space.
\end{enumerate}
We will see in Sec. \ref{sec:methods} that explicit regularization leads to iterative optimization schemes that regularize the entire solution $u$ and that implicit regularization leads to schemes that regularize only the update computed via back-propagation.

Following this convention, using a total variation regularizer \cite{mahendran2016visualizing} and blurring the pre-image $u$ with Gaussian filters \cite{oygard2015glasses,mordvintsev2015inceptionism} or bilateral filters \cite{tyka2016art} rather corresponds to an explicit regularization strategy.
In contrast to this, while blurring the update \cite{nguyen2015deep}, using of multiscale representations \cite{mordvintsev2016deepdream} or trained and untrained convolutional networks and auto-encoders \cite{dosovitskiy2015inverting,nguyen2016synthesizing,nguyen2016plug,ulyanov2017practical} corresponds rather to the second strategy.
These observation leads to the overview presented in Tab.~\ref{tab:relwork}.
In Sec.~\ref{sec:methods}, we will discuss most of these strategies, \ie total variation regularization in Sec.~\ref{s



\input{tab_related_work}


It is worth noting that Kuka{\v{c}}ka, Golkov, and Cremers 


we wish to distinguish between approaches features learning-based priors, \eg.  
So far, several regularization strategies have been proposed for obtained

focus on Regularization strategies

competitors Gaussian blur and TV

Sobolev compromise between them good regulairization with over-smoothing and easy to implement

